Galactica: A Large Language Model for Science

Information overload is a major obstacle to scientific progress. The explosive growth in scientific literature and data has made it ever harder to discover useful insights in a large mass of information. Today scientific knowledge is accessed through search engines, but they are unable to organize scientific knowledge alone. In this paper we introduce Galactica: a large language model that can store, combine and reason about scientific knowledge. We train on a large scientific corpus of papers, reference material, knowledge bases and many other sources. We outperform existing models on a range of scientific tasks. On technical knowledge probes such as LaTeX equations, Galactica outperforms the latest GPT-3 by 68.2% versus 49.0%. Galactica also performs well on reasoning, outperforming Chinchilla on mathematical MMLU by 41.3% to 35.7%, and PaLM 540B on MATH with a score of 20.4% versus 8.8%. It also sets a new state-of-the-art on downstream tasks such as PubMedQA and MedMCQA dev of 77.6% and 52.9%. And despite not being trained on a general corpus, Galactica outperforms BLOOM and OPT-175B on BIG-bench. We believe these results demonstrate the potential for language models as a new interface for science. We open source the model for the benefit of the scientific community.

==> name.tex <==
# Q108U0 (CFTR_LOXAF)

## Summary

**Protein**: Cystic fibrosis transmembrane conductance regulator

**Gene**: CFTR

**Organism**: Loxodonta africana (African elephant)

**Status**: inferred from homology

## Function

Epithelial ion channel that plays an important role in the regulation of epithelial ion and water transport and fluid homeostasis. Mediates the transport of chloride ions across the cell membrane (By similarity). Channel activity is coupled to ATP hydrolysis. The ion channel is also permeable to HCO(3-); selectivity depends on the extracellular chloride concentration. Exerts its function also by modulating the activity of other ion channels and transporters. Contributes to the regulation of the pH and the ion content of the epithelial fluid layer. Modulates the activity of the epithelial sodium channel (ENaC) complex, in part by regulating the cell surface expression of the ENaC complex. May regulate bicarbonate secretion and salvage in epithelial cells by regulating the transporter SLC4A7. Can inhibit the chloride channel activity of ANO1 (By similarity). Plays a role in the chloride and bicarbonate homeostasis during sperm epididymal maturation and capacitation (By similarity).

### Catalytic Activity

- ATP + H(2)O + closed Cl(-) channel = ADP + phosphate + open Cl(-) channel.

## Names & Taxonomy

### Protein Names

**Recommended Name:** Cystic fibrosis transmembrane conductance regulator (CFTR)

**Alternative Names:** ATP-binding cassette sub-family C member 7, Channel conductance-controlling ATPase, cAMP-dependent chloride channel

### Gene Names

**Name:** CFTR

**Synonyms:** ABCC7

### Organism

Loxodonta africana (African elephant)

### Taxonomic Identifier

NCBI Taxonomy (9785)

### Taxonomic Lineage

Eukaryota > Metazoa > Chordata > Craniata > Vertebrata > Euteleostomi > Mammalia > Eutheria > Afrotheria > Proboscidea > Elephantidae > Loxodonta

## Subcellular Location

- Apical cell membrane (location), Multi-pass membrane protein (topology)
- Early endosome membrane (location), Multi-pass membrane protein (topology)
- Cell membrane (location), Multi-pass membrane protein (topology)
- Recycling endosome membrane (location), Multi-pass membrane protein (topology)
- Endoplasmic reticulum membrane (location), Multi-pass membrane protein (topology)
- Nucleus (location)

The channel is internalized from the cell surface into an endosomal recycling compartment, from where it is recycled to the cell membrane. In the oviduct and bronchus, detected on the apical side of epithelial cells, but not associated with cilia. In Sertoli cells, a processed product is detected in the nucleus. ER stress induces GORASP2-mediated unconventional (ER/Golgi-independent) trafficking of core-glycosylated CFTR to cell membrane.

## PTM / Processing

### Features & Molecule Processing

Here are the features of the sequence for Cystic fibrosis transmembrane conductance regulator:

| Feature key | Position | Description
| --- | ----------- | --- |
| chain | 1-1482 | Cystic fibrosis transmembrane conductance regulator
| topological domain | 1-77 | Cytoplasmic
| transmembrane region | 78-98 | Helical; Name=1
| topological domain | 99-122 | Extracellular
| transmembrane region | 123-146 | Helical; Name=2
| topological domain | 147-195 | Cytoplasmic
| transmembrane region | 196-216 | Helical; Name=3
| topological domain | 217-222 | Extracellular
| transmembrane region | 223-243 | Helical; Name=4
| topological domain | 244-298 | Cytoplasmic
| transmembrane region | 299-319 | Helical; Name=5
| topological domain | 320-339 | Extracellular
| transmembrane region | 340-358 | Helical; Name=6
| topological domain | 359-858 | Cytoplasmic
| transmembrane region | 859-879 | Helical; Name=7
| topological domain | 880-919 | Extracellular
| transmembrane region | 920-940 | Discontinuously helical; Name=8
| topological domain | 941-991 | Cytoplasmic
| transmembrane region | 992-1012 | Helical; Name=9
| topological domain | 1013-1014 | Extracellular
| transmembrane region | 1015-1035 | Helical; Name=10
| topological domain | 1036-1096 | Cytoplasmic
| transmembrane region | 1097-1117 | Helical; Name=11
| topological domain | 1118-1131 | Extracellular
| transmembrane region | 1132-1152 | Helical; Name=12
| topological domain | 1153-1482 | Cytoplasmic
| domain | 81-365 | ABC transmembrane type-1 1
| domain | 423-646 | ABC transporter 1
| domain | 859-1156 | ABC transmembrane type-1 2
| domain | 1212-1445 | ABC transporter 2
| nucleotide phosphate-binding region | 458-465 | ATP
| nucleotide phosphate-binding region | 458-465 | ATP 1
| nucleotide phosphate-binding region | 1246-1253 | ATP
| nucleotide phosphate-binding region | 1246-1253 | ATP 2
| region of interest | 654-831 | Disordered R region
| region of interest | 1388-1482 | Interaction with GORASP2
| region of interest | 1454-1482 | Disordered
| short sequence motif | 1480-1482 | PDZ-binding
| compositionally biased region | 1464-1482 | Basic and acidic residues
| binding site | 401 | ATP 1
| binding site | 434 | ATP 1
| binding site | 493 | ATP 1
| binding site | 1221 | ATP 2
| modified residue | 549 | Phosphoserine
| modified residue | 660 | Phosphoserine
| modified residue | 670 | Phosphoserine; by PKA
| modified residue | 685 | Phosphoserine
| modified residue | 699 | Phosphoserine
| modified residue | 711 | Phosphoserine
| modified residue | 716 | Phosphothreonine
| modified residue | 736 | Phosphoserine
| modified residue | 767 | Phosphoserine
| modified residue | 790 | Phosphoserine
| modified residue | 795 | Phosphoserine
| modified residue | 813 | Phosphoserine
| modified residue | 1458 | Phosphoserine
| lipid moiety-binding region | 524 | S-palmitoyl cysteine
| lipid moiety-binding region | 1397 | S-palmitoyl cysteine
| glycosylation site | 894 | N-linked (GlcNAc...) asparagine
| glycosylation site | 895 | N-linked (GlcNAc...) asparagine
| glycosylation site | 901 | N-linked (GlcNAc...) asparagine
| glycosylation site | 910 | N-linked (GlcNAc...) asparagine
| cross-link | 687 | Glycyl lysine isopeptide (Lys-Gly) (interchain with G-Cter in ubiquitin)

### Post-translational modification

N-glycosylated., Phosphorylated; cAMP treatment promotes phosphorylation and activates the channel. Dephosphorylation decreases the ATPase activity (in vitro). Phosphorylation at PKA sites activates the channel. Phosphorylation at PKC sites enhances the response to phosphorylation by PKA. Phosphorylated by AMPK; this inhibits channel activity., Ubiquitinated, leading to its degradation in the lysosome. Deubiquitination by USP10 in early endosomes enhances its endocytic recycling to the cell membrane. Ubiquitinated by RNF185 during ER stress.

## Interaction

### Subunit structure

- Monomer; does not require oligomerization for channel activity. May form oligomers in the membrane (By similarity). Interacts with SLC26A3, SLC26A6 and SLC9A3R1 (By similarity). Interacts with SHANK2 (By similarity). Interacts with MYO6 (By similarity). Interacts (via C-terminus) with GOPC (via PDZ domain); this promotes CFTR internalization and thereby decreases channel activity. Interacts with SLC4A7 through SLC9A3R1. Found in a complex with MYO5B and RAB11A. Interacts with ANO1. Interacts with SLC26A8 (By similarity). Interacts with AHCYL1; the interaction increases CFTR activity (By similarity). Interacts with CSE1L (By similarity). The core-glycosylated form interacts with GORASP2 (via PDZ GRASP-type 1 domain) in respone to ER stress (By similarity).

## Family & Domains

### Domain

- Binds and hydrolyzes ATP via the two cytoplasmic ABC transporter nucleotide-binding domains. The two ATP-binding domains interact with each other, forming a head-to-tail dimer. Normal ATPase activity requires interaction between the two domains. The first ABC transporter nucleotide-binding domain has no ATPase activity by itself.
- The PDZ-binding motif mediates interactions with GOPC and with the SLC4A7, SLC9A3R1/EBP50 complex.
- The disordered R region mediates channel activation when it is phosphorylated, but not in the absence of phosphorylation.

### Sequence Similarities

- Belongs to the ABC transporter superfamily. ABCC family. CFTR transporter (TC 3.A.1.202) subfamily.

## Sequence

Here is the amino acid sequence for Cystic fibrosis transmembrane conductance regulator:

[START_AMINO]MQKSPLERASVISKLFFSWPGPILRKGYRQHLKLSDIYQIPSVDSADNLSEKLEREWDRELASKKNPKLINALRRCFFWRFVFYGILLYLGEVTKAVQPLLLGRIIASYDPDNKVERSIAIYLAIGLCLLFIVRTLLLHPAIFGLHHMGMQMRIAMFSLIYKKTLKLSSRVLDKISIGQLVSLLSNNLNKFDEGLALAHFVWIAPLQVTLLMGLIWDLLQASAFCGLAFLIIVALGQAGLGRMMMKYRDKRAGKINERLVITSEMIENIQSVKAYCWEEAMEKMIENLRQIELRLTRKAAYVRYFNSAAFFFSGFFVVFLSVLPYAMLKGIILRKIFTTISFCIVLRMAVTRQFPWAVQTWYDSLGAINKIQDFLQKQEYKTLEYNLTTTDVVMENVTAFWEEGFGELFEKAKQNNNNREISNGDNSLFFSNFSLLGAPVLKDINFKIERGQLLAVAGSTGAGKTSLLMMIMGELEPSEGKIKHSGRISFCSQFSWIMPGTIKENIIFGVSYDEYRYRSVIKACQLEEDISKFAEKDNIVLGEGGITLSGGQRARISLARAVYKDADLYLLDSPFGYLDVLTEKEIFESCVCKLMANKTRILVTSKMEHLKKADKILILHEGSSYFYGTFSELQTLRPDFSSELMGYDSFDQFSAERRNSILTETLRRFSLEGDTVSWNETKKQSFKQAGEFGEKRKNSILNSINSIRKFSVVQKTPLQMNGIDEDSDEPLERRLSLVPDSEQGEAILPRSNVINTGPTFQRRRRQSVLNLMTRPSINQGQNIHRRTAASARKMSLAPQANLTEMDIYSRRLSQDSGLEISEEINEEDLKECFFDDVENMPPVTTWNTYLRYVTVHKSLIFVLIWCLVVFLAEVAVSLVVLYLLRTSSLQDKGNNTTVNANSSYGVIVTNTSSYYLLYIYVGIADSLFALAIFRGLPLVHTLIKVSKTLHHKMLRSILQAPMSTFNTLKAGRILNRFSKDIAILDDLLPLTMFDFIQLLLIVIGAVVVVSVLQPYIFLATVPVIAAFIILRAYFLHTSQQLKQLESEARSPIFTHLVTSVKGLWTLRAFGRQPYFETLFHKALNLHTANWFLYLSTLRWFQMRIEIIFVIFFIAVTFVSILTTGEGEGTIGIILTLAMNIMNTLQWAVNSSIDVDSLMRSVSRIFKFIDMPTEESKPAKSVKPPKDGQLSKVMIIENQHVKKDYNWPSGGHMTVKDLTAKYIDGGNAILENISFSISPGQRVGLLGRTGSGKSTLLSAFLRLLNTEGEIQIDGVSWDSITLQQWRKAFGVIPQKVFIFSGTFRKNLDPYEQCSDQEIWKVADEVGLRSVIEQFPGKLDFVLVDGGYVLSHGHKQLMCLARSVLSKAKILLLDEPSAHLDPITYQIIRRTLKQAFADCTVILCEHRVEAMLECQQFLVIEENTVRQYDSIQKLLNEKSLFRQAISPLDRMKLLPHRNSSRHRSRSQIAALKEETEEEVQETRL[END_AMINO]

## Miscellaneous

### Keywords

ATP-binding, Cell membrane, Chloride, Chloride channel, Endoplasmic reticulum, Endosome, Glycoprotein, Ion channel, Ion transport, Isomerase, Isopeptide bond, Lipoprotein, Membrane, Nucleotide-binding, Nucleus, Palmitate, Phosphoprotein, Reference proteome, Repeat, Transmembrane, Transmembrane helix, Transport, Ubl conjugation

Below is the amino acid sequence for External core antigen:	[START_AMINO]MWNLRITPLSFGAACQGIFTSTLLLSALTVPLVCTIVYDSCLYMDINASRALANVYDLPDDFFPKIDDLVRDAKDALEPYWKSDSIKKHVLIATHFVDLIEDFWQTTQGMHEIAESLRAVIPPTTAPVPTGYLIQHEEAEEIPLGDLFKHQEERIVSFQPDYPITARIHAHLKAYAKINEESLDRARRLLWWHYNCLLWGEANVTNYISRLRTWLSTPEKYRGRDAPTIEAITRPIQVAQGGRKTSSGTRKPRGLEPRRRKVKTTFVYGRRRSKSRERRAPSPQRAGSPLPRSSSSHHRSPSPRK[END_AMINO]	May regulate immune response to the intracellular capsid in acting as a T-cell tolerogen, by having an immunoregulatory effect which prevents destruction of infected cells by cytotoxic T-cells.

Below is the sequence for Hepatocyte growth factor receptor:	[START_AMINO]MKAPAALAPGILVLLLTLVQKGGGECREALAKSEMNVNMRYRLPNFTADTPIQNVVVHEGHVFLGAINSIYVLRERDLQQVSEYKTGPVWEHPDCLPCQACGLAGGQWRENVNMALLVETYYDDQLISCGSVHRGTCQRHVLPRDNPADIQAEVHCMHSPRADEDEASQCPDCVVSALGTKVLLAEKQRFVNFFVGNTLNGSSLPGHALHSISVRRIKETQDGFKFLTDKSYIDVLPEFQASYPIKYIHAFESNRFIYFLTVQRETLDSPSFHTRIIRFCSADSGLRSYMEMPLECILTEKRRKRALRSEVFNVLQAAYVGKPGAQLAKQIGASAHDDILYGVFSQSRPDSAEPTDRSALCAFPVKYVDEFFHRIVNKNNVRCLQHFYGPNHLHCFNRTLLRNSSGCEVRSDEYRTEFTTALQRIDLSAGHFSQVLLTSISTFIKGDLTIANLGTSEGRFMQVVVSRSGSWTPHVDFRLDSHAVSPEVIVEHPVNQNGYTLVVTGKKITKIPLDGLGCEHFQSCSQCLSAPPFVQCGWCHDKCARAEDCPNGTWTQEICLPTIYEVFPASAPLEGGTTLTVCGWDFGFRRNNKSDFKRTRVLIGNESCPLTLSESTPNMLKCTVGPAMSEHSNLSIIISNVRGTAPQYRTFSYVDPEITSISPSYGPKAGGTLVTLTGKYLNSGNSRHISIGGKTCTLKSVSDSVLECYTPAQSISADFPVKLKIDLANREAYSFSYQENPLVVEIHPTKSFVSGGSTITVVGKNLNSVSVPRMIINVHEVEMNFTVACQQRSNSELICCTTPSLQQLDLQLPLKATAFFMLDGIHSRDFDLIYVPNPVFKLFEKPVMISMGNENVLEIKGNDIDPEAVKGEVLKVGNKSCENIHSYPESVLCTVPNDLLKLNSELNIEWKQAVSSTVLGKVIVQPDQNFTGLIVGVVSISVILLSSLGLFLWLKKRKQIKDLGSELVCYDARVHTPHLDRLVSARSVSPTTEMVSNESVDYRATFPEDQFPNSSQNGSCRQVQYPLPDLSPILTSGDSDISSPLLQNTVHIDLSALNPELVQAVQHVVIGPSSLIVHFNEVIGRGHFGCVYHGTLLDNDDRKIHCAVKSLNRITDIGEVSQFLTEGIIMKDFSHPNVLSLLGICLRSEGSPLVVLPYMKHGDLRNFIRNETHSPTVKDLIGFGLQVAKGMKYLASKKFVHRDLAARNCMLDGKFTVKVADFGLARDMYDKEYYSVHNKTGAKLPVKWMALESLQTQKFTTKSDVWSFGVLLWELMTRGAPPYPDVNTFDITVYLLQGRRLLQPEYCPDPLYEVMLKCWHPKAEMRPSFTELVSRISAIFSTFIGEHYVHVNATYVNVKCVAPYPSLLSSHDTVDGEVDT[END_AMINO]	Receptor tyrosine kinase that transduces signals from the extracellular matrix into the cytoplasm by binding to hepatocyte growth factor/HGF ligand. Regulates many physiological processes including proliferation, scattering, morphogenesis and survival. Ligand binding at the cell surface induces autophosphorylation of MET on its intracellular domain that provides docking sites for downstream signaling molecules. Following activation by ligand, interacts with the PI3-kinase subunit PIK3R1, PLCG1, SRC, GRB2, STAT3 or the adapter GAB1. Recruitment of these downstream effectors by MET leads to the activation of several signaling cascades including the RAS-ERK, PI3 kinase-AKT, or PLCgamma-PKC. The RAS-ERK activation is associated with the morphogenetic effects while PI3K/AKT coordinates prosurvival effects. During embryonic development, MET signaling plays a role in gastrulation, development and migration of muscles and neuronal precursors, angiogenesis and kidney formation. In adults, participates in wound healing as well as organ regeneration and tissue remodeling. Promotes also differentiation and proliferation of hematopoietic cells (By similarity).

[START_AMINO]MLEICLKLVGCKSKKGLSSSSSCYLEEALQRPVASDFEPQGLSEAARWNSKENLLAGPSENDPNLFVALYDFVASGDNTLSITKGEKLRVLGYNHNGEWCEAQTKNGQGWVPSNYITPVNSLEKHSWYHGPVSRNAAEYLLSSGINGSFLVRESESSPGQRSISLRYEGRVYHYRINTASDGKLYVSSESRFNTLAELVHHHSTVADGLITTLHYPAPKRNKPTVYGVSPNYDKWEMERTDITMKHKLGGGQYGEVYEGVWKKYSLTVAVKTLKEDTMEVEEFLKEAAVMKEIKHPNLVQLLGVCTREPPFYIITEFMTYGNLLDYLRECNRQEVNAVVLLYMATQISSAMEYLEKKNFIHRDLAARNCLVGENHLVKVADFGLSRLMTGDTYTAHAGAKFPIKWTAPESLAYNKFSIKSDVWAFGVLLWEIATYGMSPYPGIDLSQVYELLEKDYRMERPEGCPEKVYELMRACWQWNPSDRPSFAEIHQAFETMFQESSISDEVEKELGKQGVRGAVSTLLQAPELPTKTRTSRRAAEHRDTTDVPEMPHSKGQGESDPLDHEPAVSPLLPRKERGPPEGGLNEDERLLPKDKKTNLFSALIKKKKKTAPTPPKRSSSFREMDGQPERRGAGEEEGRDISNGALAFTPLDTADPAKSPKPSNGAGVPNGALRESGGSGFRSPHLWKKSSTLTSSRLATGEEEGGGSSSKRFLRSCSASCVPHGAKDTEWRSVTLPRDLQSTGRQFDSSTFGGHKSEKPALPRKRAGENRSDQVTRGTVTPPPRLVKKNEEAADEVFKDIMESSPGSSPPNLTPKPLRRQVTVAPASGLPHKEEAGKGSALGTPAAAEPVTPTSKAGSGAPGGTSKGPAEESRVRRHKHSSESPGRDKGKLSRLKPAPPPPPAASAGKAGGKPSQSPSQEAAGEAVLGAKTKATSLVDAVNSDAAKPSQPGEGLKKPVLPATPKPQSAKPSGTPISPAPVPSTLPSASSALAGDQPSSTAFIPLISTRVSLRKTRQPPERIASGAITKGVVLDSTEALCLAISRNSEQMASHSAVLEAGKNLYTFCVSYVDSIQQMRNKFAFREAINKLENNLRELQICPATAGSGPAATQDFSKLLSSVKEISDIVQR[END_AMINO]

[START_I_SMILES]O1[C@@H]([C@@H](O)[C@@H](O)[C@@H]1N2C(=O)NC(=O)C=C2)CCC(=O)NCC=3OC=CC3[END_I_SMILES]

Q: What will be the docking score of this compound against the protein?

Answer: -8.8

x^{2}{\frac {d^{2}y}{dx^{2}}}+x{\frac {dy}{dx}}+\left(x^{2}-\alpha ^{2}\right)y=0

\paragraph{Scaling laws of large language models} \citet{kaplan2020scaling} investigated scaling laws of Transformer language models and first showed the scaling laws are predictive of future performance. The authors found that model size (and not shape) correlates strongly with model quality, i.e., upstream cross entropy. \citet{tay2021scale} studied the scaling properties of encoder-decoder models and their impact on upstream and downstream finetuning tasks. Generally, \citet{tay2021scale} found that upstream perplexity and downstream quality does not always correlate. As a follow up, \citet{tay2022scaling} studied the scaling laws of different model architectures and found that inductive bias does significantly impact the scaling behavior of the model. Finally, \citet{hoffmann2022training} proposed compute-optimal models that popularized the \textit{`chinchilla'} scaling laws - an approach that aims to be predictive of the optimal amount of data given the number of model parameters. In this work, we mainly consider scaling laws over downstream performance largely because this is more reflective of a language model's usability. Since downstream performance is more important than upstream cross entropy, we advocate for future scaling studies to always incorporate downstream evaluation (and metrics) as opposed to only using cross entropy loss.  

